Three-loop corrections to Higgs boson pair production: reducible contribution

We compute three-loop corrections to the process $gg\to HH$ originating from one-particle reducible diagrams. This requires the computation of two-loop corrections to the gluon-gluon-Higgs vertex with an off-shell gluon. We describe in detail our approach to obtain semi-analytic results for the vertex form factors and present results for the two form factors contributing to Higgs boson pair production.

==> addl_refs.tex <==
@misc{progdata,
  author = "",
  date = "",
  howpublished = "\verb|https://www.ttp.kit.edu/preprints/2024/ttp24-0ZZ/|"
}

@article{sigmaI,
author = "Schneider, Carsten",
year = "2007",
month = "01",
pages = "1--36",
title = "{Symbolic summation assists combinatorics}",
volume = "56",
journal = "Seminaire Lotharingien de Combinatoire"
}

@article{sigmaII,
  author       = {Carsten Schneider},
  title        = {Term Algebras, Canonical Representations and Difference Ring Theory
                  for Symbolic Summation},
  journal      = {CoRR},
  volume       = {abs/2102.01471},
  year         = {2021},
  url          = {https://arxiv.org/abs/2102.01471},
  eprinttype    = {arXiv},
  eprint       = {2102.01471},
  timestamp    = {Tue, 09 Feb 2021 13:35:56 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2102-01471.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}


@incollection{RISC4711,
    author = {C. Schneider},
    title = {{Simplifying Multiple Sums in Difference Fields}},
    booktitle = {{Computer Algebra in Quantum Field Theory: Integration, Summation and Special Functions}},
    language = {english},
    series = {Texts and Monographs in Symbolic Computation},
    pages = {325--360},
    publisher = {Springer},
    isbn_issn = {ISBN-13: 978-3709116159},
    year = {2013},
    note = {arXiv:1304.4134 [cs.SC]},
    editor = {C. Schneider and J. Bluemlein},
    refereed = {no},
    length = {36},
    url = {https://www.doi.org/10.1007/978-3-7091-1616-6_14}
}

@inproceedings{RISC4826,
    author = {J. Ablinger and J. Blümlein and P. Marquard and N. Rana and C. Schneider},
    title = {{Three loop QCD corrections to heavy quark form factors}},
    booktitle = {{Proc. ACAT 2019}},
    language = {english},
    series = {J. Phys.: Conf. Ser.},
    volume = {1525},
    pages = {1--10},
    isbn_issn = {ISSN 1742-6596},
    year = {2020},
    note = {arXiv:1905.03728 [hep-ph]},
    editor = {?},
    refereed = {yes},
    length = {10},
    url = {https://www.doi.org/10.1088/1742-6596/1525/1/012018}
}
